Online Efficient Safety-Critical Control for Mobile Robots in Unknown Dynamic Multi-Obstacle Environments

This paper proposes a LiDAR-based goal-seeking and exploration framework, addressing the efficiency of online obstacle avoidance in unstructured environments populated with static and moving obstacles. This framework addresses two significant challenges associated with traditional dynamic control barrier functions (D-CBFs): their online construction and the diminished real-time performance caused by utilizing multiple D-CBFs. To tackle the first challenge, the framework's perception component begins with clustering point clouds via the DBSCAN algorithm, followed by encapsulating these clusters with the minimum bounding ellipses (MBEs) algorithm to create elliptical representations. By comparing the current state of MBEs with those stored from previous moments, the differentiation between static and dynamic obstacles is realized, and the Kalman filter is utilized to predict the movements of the latter. Such analysis facilitates the D-CBF's online construction for each MBE. To tackle the second challenge, we introduce buffer zones, generating Type-II D-CBFs online for each identified obstacle. Utilizing these buffer zones as activation areas substantially reduces the number of D-CBFs that need to be activated. Upon entering these buffer zones, the system prioritizes safety, autonomously navigating safe paths, and hence referred to as the exploration mode. Exiting these buffer zones triggers the system's transition to goal-seeking mode. We demonstrate that the system's states under this framework achieve safety and asymptotic stabilization. Experimental results in simulated and real-world environments have validated our framework's capability, allowing a LiDAR-equipped mobile robot to efficiently and safely reach the desired location within dynamic environments containing multiple obstacles.

==> Figs/analysis/tikz/dis_line.tex <==
\begin{tikzpicture}
\node[fill opacity=0.15] at (0,0) {\includegraphics[width=0.5\columnwidth,angle=-90,trim=50 100 50 0,clip]{Figs/analysis/robot_0.png}};

\coordinate (rl) at (-0.8,1.45);
\coordinate (fr) at (2.2,-1.1);
\coordinate (p_dis) at ($(rl)!0.325!0:(fr)$); 
\coordinate (p_dis_1) at ($(rl)!0.2!0:(fr)$);
\coordinate (com) at ($(p_dis)!0.65!90:(rl)$);

\coordinate (com_1) at ($(com)!0.6!90:(p_dis)$);
\coordinate (p_dis_1) at ($(p_dis)!0.6!-90:(com)$);

\draw[color=blue,line width=2pt,dashed](rl) -- (fr);
\draw[color=blue,line width=2pt,dashed](p_dis) -- (com);
\draw[color=blue,line width=2pt,dashed](com) -- (com_1);

\draw [gray,fill=black,opacity=0.75] (rl) circle (0.15);
\draw [gray,fill=black,opacity=0.75] (fr) circle (0.15);
\draw [gray,fill=black,opacity=1] (com) circle (0.15);
\markRightAngle {fr}{p_dis}{com};

\draw[color=red,line width=1pt,<->](p_dis_1) -- (com_1);

\node at (-0.8,1.8) {\footnotesize $P_h(hx,hy)$};
\node at (2.65,-1.45) {\footnotesize $P_f(fx,fy)$};
\node at (-0.25,-0.3) {\footnotesize $CoM(cx,cy)$};
\node at (-0.8,0.75) {\footnotesize $dis(t)$};

\coordinate (p_o) at (1,0);
\coordinate (x0) at (3,0);
\coordinate (x1) at (-2,0);
\coordinate (y0) at (1.7,1.5);
\coordinate (y1) at (1.7,-1.5);


\draw[color=black,line width=1pt,->](x1) -- (x0);
\draw[color=black,line width=1pt,->](y1) -- (y0);

\node at (3.1,0) {\footnotesize $x$};
\node at (2,1.5) {\footnotesize $y$};


\end{tikzpicture}

==> Figs/exp/tikz/env_set.tex <==
\begin{tikzpicture}
\node[fill opacity=0.5] at (0,0) {\includegraphics[width=\columnwidth,angle=-180,trim=0 500 0 750,clip]{Figs/exp/env.jpg}};

\coordinate (po) at (1,0.5);
\coordinate (px) at (-1,0);
\coordinate (py) at (2,-0.5);
\coordinate (pz) at (1,1.5);

\draw[color=blue,line width=3pt,->] (po) -- (px);
\draw[color=black,line width=3pt,->] (po) -- (py);
\draw[color=black,line width=3pt,->] (po) -- (pz);

%\node[fill=white] at (-1.1,0) {$x$};
%\node[fill=white] at (2.1,-0.5) {$y$};
%\node[fill=white] at (0.75,1.25) {$z$};
\node at (-1.1,0) {$x$};
\node at (2.1,-0.5) {$y$};
\node at (0.75,1.25) {$z$};

\node[fill=white]  at (-0.5,-0.5) {$\theta_{roll}$};
\node[fill=white]  at (1.5,-1) {$\theta_{pitch}$};

\draw[color=red,line width=2pt,->] (-0.5,0.35) arc(150:-120:0.4);
\draw[color=red,line width=2pt,->] (2,0) arc(30:300:0.4);
\end{tikzpicture}

==> Figs/exp/tikz/env_set_1.tex <==
\begin{tikzpicture}
\node[fill opacity=0.8] at (0,0) {\includegraphics[width=\columnwidth,trim=0 0 0 0 ,clip]{Figs/exp/env_3.png}};

\coordinate (po) at (0.5,-0.1);
\coordinate (px) at (2.1,-0.1);
\coordinate (py) at (0.5,1.5);

\draw[color=white, line width=4pt, ->] (2.5,-0.1) -- (4,-0.1);

\draw[color=cyan!50,line width=2pt,->] (po) -- (px);
\draw[color=cyan!50,line width=2pt,->] (po) -- (py);


\node[color=white] at (2.1,0.1) {$\mathbf{x}$};
\node[color=white] at (0.25,1.45) {$\mathbf{y}$};

\node[color=white]  at (-0.25,1) {\large $\mathbf{\theta_{pitch}}$};
\node[color=white]  at (1.5,-0.5) {\large $\mathbf{\theta_{roll}}$};

\draw[color=red!50,line width=1.5pt,-latex,dashed] (0.3,0.5) arc(210:-30:0.3);
\draw[color=red!50,line width=1.5pt,-latex,dashed] (1.8,0.2) arc(30:300:0.3);

\end{tikzpicture}

==> Figs/exp/tikz/env_set_1_0.tex <==
\begin{tikzpicture}
\node[fill opacity=0.75] at (0,0) {\includegraphics[width=0.42\columnwidth,angle=90,trim=300 0 1000 0 ,clip]{Figs/exp/env_1.jpg}};

\coordinate (po) at (-0.5,0);
\coordinate (px) at (1,0);
\coordinate (py) at (-0.5,1.5);

\draw[color=blue, line width=3pt, ->] (1.25,0) -- (2.5,0);

\draw[color=black!75,line width=2pt,->] (po) -- (px);
\draw[color=black!75,line width=2pt,->] (po) -- (py);


\node at (1.0,0.25) {$x$};
\node at (-0.25,1.5) {$y$};
\node[color=white]  at (-1.25,0.75) {\large $\mathbf{\theta_{pitch}}$};
\node[color=white]  at (0.75,-0.5) {\large $\mathbf{\theta_{roll}}$};

\draw[color=white,line width=1.5pt,-latex,dashed] (-0.7,0.5) arc(210:-30:0.3);
\draw[color=white,line width=1.5pt,-latex,dashed] (0.5,0.2) arc(30:300:0.3);

\end{tikzpicture}

==> Figs/exp/tikz/ground_foot.tex <==
\begin{tikzpicture}
\node[fill opacity=0.5] at (0,0) {\includegraphics[width=.9\columnwidth]{Figs/exp/foot.pdf}};

\coordinate (g0_1) at (-4,-1.45);
\coordinate (g0_2) at (4,-1.45);
\draw[color=black,line width=3pt] (g0_1) -- (g0_2);
\foreach \i in {0, 1, ..., 9}
{
    \draw[color=black,line width=1.5pt] (-3.2+\i*0.8,-1.45) -- (-4+\i*0.8,-1.65);
}
\end{tikzpicture}

==> Figs/exp/tikz/ground_foot_1.tex <==
\begin{tikzpicture}
\node[fill opacity=0.5] at (0,0) {\includegraphics[width=.9\columnwidth]{Figs/exp/foot_1.pdf}};

\coordinate (g0_1) at (-4,-1.25);
\coordinate (g0_2) at (4,-1.25);
\draw[color=black,line width=3pt] (g0_1) -- (g0_2);
\foreach \i in {0, 1, ..., 9}
{
    \draw[color=black,line width=1.5pt] (-3.2+\i*0.8,-1.25) -- (-4+\i*0.8,-1.45);
}
\end{tikzpicture}

==> Figs/intro/tikz/case.tex <==
\begin{tikzpicture}
%\node[fill opacity=0.9] at (0,0) %{\includegraphics[width=.9\columnwidth]{Figs/model_tikz/fig/rat_spine_v1.pdf}};

%\node[anchor=west] at (-4.5,-1.5) {\footnotesize Right fore leg (RF)};
%\node[anchor=west] at (-3,-2) {\footnotesize Left fore leg (LF)};
%\node[anchor=west] at (-1.35,-0.6) {\footnotesize Right hind leg (RH)};
%\node[anchor=west] at (0.5,-1) {\footnotesize Left hind leg (LH)};

%\node[anchor=west] at (-1.5,1.45) {\footnotesize Spine};
%\node at (-4.5,1.45)[anchor=west] {\footnotesize The motor to};
%\node at (-4.5,1.2)[anchor=west] {\footnotesize actuate the spine};
%\draw[color=red,line width=1.5pt,dashed,->](-3.2,1.1) -- (-2.2,0.9);

%\node at (0.5,1.75)[anchor=west] {\footnotesize Right hip};
%\draw[color=red,line width=1.5pt,dashed,->](0,1.5) -- (0.6,1.7);

%\node at (1.5,0.25)[anchor=west] {\footnotesize Left hip};
%\draw[color=red,line width=1.5pt,dashed,->](1,1) -- (2,0.5);


%\node at (2,1.35)[anchor=west] {\footnotesize Tail};
\coordinate (p1) at (0,0);
\coordinate (p2) at (1.5,0-0.2);
\coordinate (p3) at (2,1.5);
\coordinate (p4) at (3.5,1.5-0.2);
\coordinate (p5) at (0-0.1,-0.5);
\coordinate (p6) at (1.5-0.1,-0.5-0.2);
\coordinate (p7) at (3.5-0.1,1-0.2);

\coordinate (f5) at (0-0.2,-0.5-1);
\coordinate (f6) at (1.5-0.2,-0.5-0.2-0.5);
\coordinate (f7) at (3.5-0.2,1-0.2-1);

\coordinate (c1) at (2,0.75);
\coordinate (c2) at (2,0.75-1.75);

\draw[color=black,line width=1.5pt](p1) -- (p2);
\draw[color=black,line width=1.5pt](p3) -- (p4);
\draw[color=black,line width=1.5pt](p1) -- (p3);
\draw[color=black,line width=1.5pt](p2) -- (p4);
\draw[color=black,line width=1.5pt](p1) -- (p5);
\draw[color=black,line width=1.5pt](p2) -- (p6);
\draw[color=black,line width=1.5pt](p4) -- (p7);
\draw[color=black,line width=1.5pt](p5) -- (p6);
\draw[color=black,line width=1.5pt](p6) -- (p7);

\draw[color=black,line width=1.5pt](p5) -- (f5);
\draw[color=black,line width=1.5pt](p6) -- (f6);
\draw[color=black,line width=1.5pt](p7) -- (f7);

\draw[color=blue,line width=2pt,dashed](f5) -- (f7);

\fill[color=black] (c1) circle (5pt);
\draw[color=red,line width=1pt,dashed,->](c1) -- (c2);


\end{tikzpicture}

==> Figs/intro/tikz/case_0.tex <==
\begin{tikzpicture}
\node[fill opacity=0.9] at (-3,1) {\scalebox{1}[-1]{\includegraphics[width=.45\columnwidth,angle=180]{Figs/intro/gait.png}}};

\coordinate (f1) at (-4,0.275);
\coordinate (f2) at (-2.5,0.325);
\fill[color=blue!50, fill opacity=0.45]  (f1) ellipse [x radius=6pt, y radius=4pt];
\fill[color=blue!50, fill opacity=0.45]  (f2) ellipse [x radius=6pt, y radius=4pt];
\draw[color=blue!35,line width=2pt](f1) -- (f2);

\coordinate (rcom) at (-4,0.275);
\fill[color=black, fill opacity=0.5]  (-3.25,1.25) circle (5pt);
\draw[color=red,line width=1pt,->] (-3.25,1.25) --  (-3.25,0.75);

\draw[color=black,line width=1pt,dashed] (-1,1.5) --  (2,1.75);
\draw[color=black,line width=1pt,dashed] (-3.25,0) --  (-1,-1.5);


\coordinate (p1) at (0,0);
\coordinate (p2) at (1.5,0-0.2);
\coordinate (p3) at (2,1.5);
\coordinate (p4) at (3.5,1.5-0.2);
\coordinate (p5) at (0-0.1,-0.5);
\coordinate (p6) at (1.5-0.1,-0.5-0.2);
\coordinate (p7) at (3.5-0.1,1-0.2);

\coordinate (f5) at (0-0.2,-0.5-1);
\coordinate (f6) at (1.5-0.2,-0.5-0.2-0.5);
\coordinate (f7) at (3.5-0.2,1-0.2-1);

\coordinate (pf5) at (0,-0.5);
\coordinate (pf6) at (1.5-0.2,-0.5-0.2);
\coordinate (pf7) at (3.5-0.2,1-0.25);

\coordinate (c1) at (2,0.75);
\coordinate (c2) at (2,0.75-1.75);

\fill[color=blue!50, fill opacity=0.35]  (f5) ellipse [x radius=10pt, y radius=5pt];
\fill[color=blue!50, fill opacity=0.35]  (f7) ellipse [x radius=10pt, y radius=5pt];
\draw[color=blue!20,line width=4pt](f5) -- (f7);


\fill[color=black] (c1) circle (5pt);
\draw[color=red,line width=1pt,->](c1) -- (c2);


\fill[color=orange,fill opacity=0.55,line width=1.5pt](p1) -- (p2) -- (p4)  -- (p3) -- (p1);
\fill[color=orange,fill opacity=0.35,line width=1.5pt] (p4) -- (p2)  -- (p6) -- (p7) -- (p4);
\fill[color=orange,fill opacity=0.15,line width=1.5pt] (p1) -- (p5)  -- (p6) -- (p2) -- (p1);


\draw[color=black,line width=2pt](pf5) -- (f5);
\draw[color=black,line width=2pt](pf6) -- (f6);
\draw[color=black,line width=2pt](pf7) -- (f7);

\end{tikzpicture}

==> Figs/intro/tikz/case_1.tex <==
\begin{tikzpicture}
\node[fill opacity=0.9] at (-3,1) {\scalebox{1}[-1]{\includegraphics[width=.45\columnwidth,angle=180]{Figs/intro/gait.png}}};

\coordinate (f1) at (-4,0.275);
\coordinate (f2) at (-2.5,0.325);
\fill[color=blue!50, fill opacity=0.45]  (f1) ellipse [x radius=6pt, y radius=4pt];
\fill[color=blue!50, fill opacity=0.45]  (f2) ellipse [x radius=6pt, y radius=4pt];
\draw[color=blue!35,line width=2pt](f1) -- (f2);

\coordinate (rcom) at (-4,0.275);
\fill[color=black, fill opacity=0.5]  (-3.25,1.25) circle (5pt);
\draw[color=red,line width=1pt,->] (-3.25,1.25) --  (-3.25,0.75);

\draw[color=black,line width=1pt,dashed] (-1,1.5) --  (2,1.75);
\draw[color=black,line width=1pt,dashed] (-3.25,0) --  (-1,-1.5);


\coordinate (p1) at (0,0);
\coordinate (p2) at (1.5,0-0.2);
\coordinate (p3) at (2,1.5);
\coordinate (p4) at (3.5,1.5-0.2);
\coordinate (p5) at (0-0.1,-0.5);
\coordinate (p6) at (1.5-0.1,-0.5-0.2);
\coordinate (p7) at (3.5-0.1,1-0.2);

\coordinate (pf5) at (0,-0.5);
\coordinate (pf6) at (1.5-0.2,-0.5-0.2);
\coordinate (pf7) at (3.5-0.2,1-0.25);
\coordinate (pf8) at (2.3,0);

\coordinate (f5) at (0-0.2,-0.5-1);
%\coordinate (f6) at (1.5-0.2,-0.5-0.2-0.5);
\coordinate (f6_t) at (1.5-0.2,-0.5-0.2-0.5);
\coordinate (f6) at (1.5-0.1,-0.5-0.2-0.65);
\coordinate (f7) at (3.5-0.2,1-0.2-1);
\coordinate (f8) at (2.3,-0.25);


\coordinate (mf5) at (0,-0.5-0.5);
\coordinate (mf6) at (1.5,-0.5-0.2-0.35);
\coordinate (mf7) at (3.5-0.1,1-0.2-0.5);


\coordinate (c1) at (2,0.75);
\coordinate (c2) at (2,0.75-1.75);

\fill[color=blue!50, fill opacity=0.35]  (f5) ellipse [x radius=10pt, y radius=5pt];
\fill[color=blue!50, fill opacity=0.35]  (f7) ellipse [x radius=10pt, y radius=5pt];
\draw[color=blue!20,line width=4pt](f5) -- (f7);


\fill[color=black] (c1) circle (5pt);
\draw[color=red,line width=1pt,->](c1) -- (c2);


\fill[color=orange,fill opacity=0.55,line width=1.5pt](p1) -- (p2) -- (p4)  -- (p3) -- (p1);
\fill[color=orange,fill opacity=0.35,line width=1.5pt] (p4) -- (p2)  -- (p6) -- (p7) -- (p4);
\fill[color=orange,fill opacity=0.15,line width=1.5pt] (p1) -- (p5)  -- (p6) -- (p2) -- (p1);


\draw[color=black,line width=2pt](pf5) -- (mf5) -- (f5);
\draw[color=black,line width=2pt](pf6) -- (mf6) -- (f6);
%\draw[color=black,line width=2pt](pf6) -- (f6_t);
\draw[color=black,line width=2pt](pf7) -- (mf7) -- (f7);
\draw[color=black,line width=2pt](pf8) -- (f8);

\fill[color=black, fill opacity=0.85]  (mf5) circle (2.5pt);
\fill[color=black, fill opacity=0.85]  (mf6) circle (2.5pt);
\fill[color=black, fill opacity=0.85]  (mf7) circle (2.5pt);

\fill[color=black, fill opacity=0.85]  (f5) circle (3pt);
\fill[color=black, fill opacity=0.85]  (f6) circle (3pt);
\fill[color=black, fill opacity=0.85]  (f7) circle (3pt);
\fill[color=black, fill opacity=0.85]  (f8) circle (3pt);

\node[anchor=west] at (2,1) {\footnotesize CoM};
\node[anchor=west] at (2.4,-0.75) {\footnotesize Support};
\node[anchor=west] at (2.4,-1) {\footnotesize Area};

\end{tikzpicture}

==> Figs/model/tikz/body.tex <==
\begin{tikzpicture}
\coordinate (com) at (0,0);
\coordinate (com_0) at (0,-1);
\coordinate (com_1) at (0,0.5);
\coordinate (com_2) at (0,-0.5);

\coordinate (base0_0) at (2.5,0);
\coordinate (base0_1) at (-2.5,0);
\coordinate (base0_2) at (-2,0);
\coordinate (base1_0) at ($(com)!1!10:(base0_0)$);
\coordinate (base2_0) at ($(com)!-1!10:(base0_0)$);
\coordinate (base3_0) at ($(com)!0.5!90:(base1_0)$);
\coordinate (base1) at ($(com)!0.6!10:(base0_0)$);
\coordinate (base2) at ($(com)!-0.6!10:(base0_0)$);

\coordinate (p1) at ($(base1)!0.1!90:(base2)$);
\coordinate (p2) at ($(base1)!-0.1!90:(base2)$);
\coordinate (p3) at ($(base2)!0.1!90:(base1)$);
\coordinate (p4) at ($(base2)!-0.1!90:(base1)$);

\gettikzxy{(p1)}{\pxr}{\pyr};
\gettikzxy{(p4)}{\pxl}{\pyl};
\coordinate (f1) at (\pxr,-1.5);
\coordinate (f4) at (\pxl,-1.5);

\coordinate (g0_1) at (-2.5,-1.5);
\coordinate (g0_2) at (2.5,-1.5);

\draw[color=red,line width=1pt,->](com) -- (com_0);
\draw[color=black,line width=1pt,dashed] (base0_0) -- (base0_1);
\draw[color=black,line width=1pt,<-] (base1_0) -- (base2_0);
\draw[color=black,line width=1pt,->] (com) -- (base3_0);
\draw[color=black,line width=1pt] (base2) -- (p3);
\draw[color=black,line width=1pt] (base2) -- (p4);
\draw[color=gray,line width=2pt] (p1) -- (p2) -- (p3) -- (p4) -- (p1);
\draw[color=gray,line width=2pt] (p1) -- (f1);
\draw[color=gray,line width=2pt] (p4) -- (f4);

\draw[color=black,line width=1pt] (base0_2) arc(-180:-170:2);
\draw[color=black,line width=2pt] (g0_1) -- (g0_2);
\foreach \i in {0, 1, ..., 9}
{
    \draw[color=black,line width=1pt] (-2+\i*0.5,-1.5) -- (-2.5+\i*0.5,-1.75);
}

\node at (-2.5,-0.2) {\footnotesize $\theta_{roll}$};
\node at (0,1.25) {$\mathbf{z}$};
\node at (2.5,0.25) {$\mathbf{y}$};

\node at (-2,-1.25) {\footnotesize $RH$};
\node at (2,-1.25) {\footnotesize $LF$};

\end{tikzpicture}

==> Figs/model/tikz/dis_period.tex <==
\begin{tikzpicture}
\node[fill opacity=0.15] at (0,0) {\includegraphics[width=\columnwidth]{Figs/model/dis.pdf}};
%{\includegraphics[width=\columnwidth]{Figs/model/dis_t.pdf}};

\coordinate (line_0) at (-3,0.3);
\coordinate (line_1) at (4.2,0.3);
\coordinate (area_0) at (-3,1.6);
\coordinate (area_1) at (-3,-1);

\fill[cyan, opacity=0.1] (area_0) rectangle (line_1);
\fill[magenta, opacity=0.1] (area_1) rectangle (line_1);

\draw[color=red,line width=2pt,dashed] (area_1) rectangle (-1,1.6);

\node at (3.8,1.35) {\textbf{Right}};
\node at (3.9,-0.05) {\textbf{Left}};
\end{tikzpicture}

==> Figs/model/tikz/dis_period_1.tex <==
\begin{tikzpicture}
\node[fill opacity=0.15] at (0,0) {\includegraphics[width=\columnwidth,trim=0 0 0 0,clip]{Figs/model/fig1.pdf}};
\node[fill opacity=0.15] at (0,0) {\includegraphics[width=\columnwidth,trim=0 0 0 0,clip]{Figs/model/fig2.pdf}};
\node[fill opacity=0.15] at (0,0) {\includegraphics[width=\columnwidth,trim=0 0 0 0,clip]{Figs/model/fig3.pdf}};
\node[fill opacity=0.15] at (0,0) {\includegraphics[width=\columnwidth,trim=0 0 0 0,clip]{Figs/model/fig8.pdf}};
\node[fill opacity=0.15] at (0,0) {\includegraphics[width=\columnwidth,trim=0 0 0 0,clip]{Figs/model/fig10.pdf}};
\node[fill opacity=0.15] at (0,0) {\includegraphics[width=\columnwidth,trim=0 0 0 0,clip]{Figs/model/fig11.pdf}};
\end{tikzpicture}

==> Figs/model/tikz/state.tex <==
\begin{tikzpicture}
\coordinate (s0) at (-2,0);
\coordinate (s1) at (2,0);

%\draw [gray,opacity=1] (s0) circle (1.25);
\draw [gray,opacity=1,line width=2pt] (s0) ellipse [x radius=1.25, y radius=0.75];
%\draw [gray,opacity=1] (s1) circle (1.25);
\draw [gray,opacity=1,line width=2pt] (s1) ellipse [x radius=1.25, y radius=0.75];

\draw[color=black,line width=2pt,->] (-1,0.5) arc(110:70:3);
\draw[color=black,line width=2pt,->] (1,-0.5) arc(-70:-110:3);



\node at (-2.75,0.25) {$k=$};
\node at (-2,-0.25) {\footnotesize $\frac{2\arccos{\frac{R'}{\alpha}}}{\pi}$};
\node at (1.25,0.25) {$k=$};
\node at (2,-0.25) {\footnotesize $2-\frac{2\arccos{\frac{R'}{\alpha}}}{\pi}$};

\node at (0,1) {\footnotesize $t=\frac{(2n+1)T}{4}$};
\node at (0,-1) {\footnotesize $t=\frac{nT}{2}$};

\end{tikzpicture}

==> Figs/old/exp_tikz/cases.tex <==
\begin{tikzpicture}
\node[fill opacity=0.4] at (0,0) {\includegraphics[width=0.41\columnwidth]{Figs/exp_tikz/fig/cases.pdf}};

\node at (-0.8,0.75) {\footnotesize Case 1};
\node at (0.6,0.25) {\footnotesize Case 2};
\end{tikzpicture}

==> Figs/old/exp_tikz/env.tex <==
\begin{tikzpicture}
\node[fill opacity=0.4] at (0,0) {\includegraphics[width=0.435\columnwidth]{Figs/exp_tikz/fig/env.pdf}};

\node at (-1.75,0.2) {\footnotesize $x$};
\node at (-1.1,0.5) {\footnotesize $y$};
\node at (-1.6,0.75) {\footnotesize $z$};


\end{tikzpicture}

==> Figs/old/exp_tikz/real_res.tex <==
\begin{tikzpicture}
\node[fill opacity=1] at (-7,0) {\includegraphics[width=0.4\columnwidth]{Figs/exp_tikz/real/t0.png}};
\node[fill opacity=1] at (-3.5,0) {\includegraphics[width=0.4\columnwidth]{Figs/exp_tikz/real/t3.png}};
\node[fill opacity=1] at (0,0) {\includegraphics[width=0.4\columnwidth]{Figs/exp_tikz/real/t6.png}};
\node[fill opacity=1] at (3.5,0) {\includegraphics[width=0.4\columnwidth]{Figs/exp_tikz/real/t9.png}};
\node[fill opacity=1] at (7,0) {\includegraphics[width=0.4\columnwidth]{Figs/exp_tikz/real/t12.png}};

%\fill[white] (-1.25,-1) rectangle (-1.75,-0.5);
%\node at (-1.5,-0.85) {\footnotesize 0T};
%\draw[color=red,line width=1.5pt,dashed,->](1,1) -- (2,0.5);

\fill[white] (-8.75,1.75) rectangle (-7.75,1.25);
\node at (-8.25,1.5) {\footnotesize t = 0s};

\fill[white] (-5.25,1.75) rectangle (-4.25,1.25);
\node at (-4.75,1.5) {\footnotesize t = 3s};

\fill[white] (-1.75,1.75) rectangle (-0.75,1.25);
\node at (-1.25,1.5) {\footnotesize t = 6s};

\fill[white] (1.75,1.75) rectangle (2.75,1.25);
\node at (2.25,1.5) {\footnotesize t = 9s};

\fill[white] (5.25,1.75) rectangle (6.25,1.25);
\node at (5.75,1.5) {\footnotesize t = 12s};

\end{tikzpicture}

==> Figs/old/model_tikz/rat.tex <==
\begin{tikzpicture}
\node[fill opacity=0.9] at (0,0) {\includegraphics[width=.9\columnwidth]{Figs/model_tikz/fig/rat_spine_v1.pdf}};

\node[anchor=west] at (-4.5,-1.5) {\footnotesize Right fore leg (RF)};
\node[anchor=west] at (-3,-2) {\footnotesize Left fore leg (LF)};
\node[anchor=west] at (-1.35,-0.6) {\footnotesize Right hind leg (RH)};
\node[anchor=west] at (0.5,-1) {\footnotesize Left hind leg (LH)};

\node[anchor=west] at (-1.5,1.45) {\footnotesize Spine};
\node at (-4.5,1.45)[anchor=west] {\footnotesize The motor to};
\node at (-4.5,1.2)[anchor=west] {\footnotesize actuate the spine};
\draw[color=red,line width=1.5pt,dashed,->](-3.2,1.1) -- (-2.2,0.9);

\node at (0.5,1.75)[anchor=west] {\footnotesize Right hip};
\draw[color=red,line width=1.5pt,dashed,->](0,1.5) -- (0.6,1.7);

\node at (1.5,0.25)[anchor=west] {\footnotesize Left hip};
\draw[color=red,line width=1.5pt,dashed,->](1,1) -- (2,0.5);


\node at (2,1.35)[anchor=west] {\footnotesize Tail};

\end{tikzpicture}

==> Figs/old/model_tikz/swing_0.tex <==
\begin{tikzpicture}
\node[fill opacity=0.4] at (0,0) {\includegraphics[width=0.3\columnwidth]{Figs/model_tikz/fig/0.png}};

\node[anchor=west] at (-4,2.5) {\footnotesize Support phases};
\draw[color=blue,opacity=0.6,line width=1.5pt,->](-4,2) -- (-3,2);

\node[anchor=west] at (-4,1.5) {\footnotesize Swing phases};
\draw[color=red,opacity=0.6,line width=1.5pt,->](-4,1) -- (-3,1);

\node[anchor=west] at (-4,0.5) {\footnotesize Spinal swing direction};
\draw[color=blue,opacity=0.6,line width=2pt,dashed,->](-4,0) -- (-3,0);

\draw[color=blue,opacity=0.6,line width=1.5pt,dashed,->] (-0.25,0) arc (180:270:0.5);

\draw[color=blue,opacity=0.6,line width=1.5pt,->](-0.9,0) -- (-0.9,-0.5);
\draw[color=red,opacity=0.6,line width=1.5pt,->](0.25,-1.5) -- (0.25,-1);

\end{tikzpicture}

==> Figs/old/model_tikz/swing_1.tex <==
\begin{tikzpicture}
\node[fill opacity=0.4] at (0,0) {\includegraphics[width=0.3\columnwidth]{Figs/model_tikz/fig/1.png}};


\draw[color=blue,opacity=0.6,line width=1.5pt,dashed,->] (-0.25,0) arc (180:270:0.5);

\draw[color=blue,opacity=0.6,line width=1.5pt,->](-0.9,0) -- (-0.9,-0.5);
\draw[color=red,opacity=0.6,line width=1.5pt,->](0.5,-1.25) -- (0.5,-0.75);

\end{tikzpicture}

==> Figs/old/model_tikz/swing_2.tex <==
\begin{tikzpicture}
\node[fill opacity=0.4] at (0,0) {\includegraphics[width=0.3\columnwidth]{Figs/model_tikz/fig/2.png}};


\draw[color=blue,opacity=0.6,line width=1.5pt,dashed,->] (-0.25,0) arc (180:270:0.5);

\draw[color=blue,opacity=0.6,line width=1.5pt,->](-0.25,-1) -- (-0.25,-1.5);
\draw[color=red,opacity=0.6,line width=1.5pt,->](0.9,-0.25) -- (0.9,0.25);

\end{tikzpicture}

==> Figs/old/model_tikz/swing_3.tex <==
\begin{tikzpicture}
\node[fill opacity=0.4] at (0,0) {\includegraphics[width=0.3\columnwidth]{Figs/model_tikz/fig/2.png}};

\draw[color=blue,opacity=0.6,line width=1.5pt,dashed,->] (0.25,0) arc (0:-90:0.5);

\draw[color=blue,opacity=0.6,line width=1.5pt,->](0.9,0) -- (0.9,-0.5);
\draw[color=red,opacity=0.6,line width=1.5pt,->](-0.25,-1.5) -- (-0.25,-1);

\end{tikzpicture}

==> Figs/old/model_tikz/topo.tex <==
\begin{tikzpicture}
\node[fill opacity=0.9] at (0,0) {\includegraphics[width=.9\columnwidth]{Figs/model_tikz/fig/topo_v1.pdf}};

\fill[white] (-3.5,0.1) rectangle (-3,-0.25);
\node at (-3.3,0) {\footnotesize 0.5T};
\fill[white] (-2.5,0.1) rectangle (-2,-0.25);
\node at (-2.3,0) {\footnotesize -0.5T};

\fill[white] (3,0.1) rectangle (3.5,-0.25);
\node at (3.4,0) {\footnotesize 0.5T};
\fill[white] (2,0.1) rectangle (2.5,-0.25);
\node at (2.4,0) {\footnotesize -0.5T};

%\fill[white] (-0.35,0.25) rectangle (0.25,0.5);
\node at (0,0.3) {\footnotesize 0.5T};
%\fill[white] (-0.35,-0.45) rectangle (0.25,-0.75);
\node at (0,-0.3) {\footnotesize -0.5T};

\fill[white] (1.25,1) rectangle (1.75,0.5);
\node at (1.5,0.85) {\footnotesize 0.5T};
\fill[white] (-1.25,1) rectangle (-1.75,0.5);
\node at (-1.5,0.85) {\footnotesize 0.5T};
\fill[white] (1.25,-1) rectangle (1.75,-0.5);
\node at (1.5,-0.85) {\footnotesize 0T};
\fill[white] (-1.25,-1) rectangle (-1.75,-0.5);
\node at (-1.5,-0.85) {\footnotesize 0T};

\node at (-2.75,-1.9) {\footnotesize${CPG}_{LH}$};
\node at (-2.75,1.9) {\footnotesize${CPG}_{LF}$};
\node at (3,-1.9) {\footnotesize${CPG}_{RH}$};
\node at (3,1.9) {\footnotesize${CPG}_{RF}$};
\node at (-0.6,-0.8) {\footnotesize${CPG}_{LS}$};
\node at (0.6,0.8) {\footnotesize${CPG}_{RS}$};


\end{tikzpicture}
